Brightening the Optical Flow through Posit Arithmetic

As new technologies are invented, their commercial viability needs to be carefully examined along with their technical merits and demerits. The posit data format, proposed as a drop-in replacement for IEEE 754 float format, is one such invention that requires extensive theoretical and experimental study to identify products that can benefit from the advantages of posits for specific market segments. In this paper, we present an extensive empirical study of posit-based arithmetic vis-\`a-vis IEEE 754 compliant arithmetic for the optical flow estimation method called Lucas-Kanade (LuKa). First, we use SoftPosit and SoftFloat format emulators to perform an empirical error analysis of the LuKa method. Our study shows that the average error in LuKa with SoftPosit is an order of magnitude lower than LuKa with SoftFloat. We then present the integration of the hardware implementation of a posit adder and multiplier in a RISC-V open-source platform. We make several recommendations, along with the analysis of LuKa in the RISC-V context, for future generation platforms incorporating posit arithmetic units.

==> rw.tex <==
Since the inception of posit data representation and arithmetic, there have been several implementations in the literature of posit operations. The early and open-source hardware implementations of posit adder and multiplier were presented in \cite{posit1} and \cite{posit2}. In \cite{posit2}, the authors covered design of a parametric adder/subtractor while in \cite{posit1}, the authors presented parametric designs of float-to-posit and posit-to-float converters, and a multiplier along with the design of an adder/subtractor. A major disadvantage of the designs presented in \cite{posit1} and \cite{posit2} is that the designs are yet to be fully verified and contain multiple errors. %....\#\#\#\#\#Mention one bug here\#\#\#\#\#\#\#\#
The PACoGen open-source framework that can generate pipelined adder/subtractor, multiplier, and divider is presented in \cite{posit3}. PACoGen is capable of generating hardware units that can adapt precision at run time. The design presented in \cite{posit3} has a disadvantage similar to those presented in \cite{posit2} and \cite{posit1}. A more reliable implementation of a parametric posit adder and multiplier generator is presented in \cite{iccd1}. A major drawback of the generator presented in \cite{iccd1} is that it is non-pipelined design, which results in a low operating frequency for large bit-width adders and multipliers. 

\emph{Cheetah}, presented in \cite{langroudi2019cheetah}, discusses deep neural network (DNN) training using posits. However, we believe that the architecture presented in \cite{langroudi2019cheetah} is over-designed and can be greatly optimized. Also, the comparison for DNN benchmarks in \cite{langroudi2019cheetah} is easy to create with the test-bed that we provide. Apart from the mentioned efforts, there have been several other implementations of posit hardware units \cite{iscas1, zhang1}. To the best of our knowledge, this is the first-ever industrial case-study for posits incorporating RISC-V integration. 
 
